Saharaline: A Collective Social Support Intervention for Teachers in Low-Income Indian Schools

This paper presents Saharaline, an intervention designed to provide collective social support for teachers in low-income schools. Implemented as a WhatsApp-based helpline, Saharaline enables teachers to reach out for personalized, long-term assistance with a wide range of problems and stressors, including pedagogical, emotional, and technological challenges. Depending on the support needed, teachers' requests are routed to appropriate domain experts -- staff employed by educational non-profit organizations who understand teachers' on-the-ground realities -- who offer localized and contextualized assistance. Via a three-month exploratory deployment with 28 teachers in India, we show how Saharaline's design enabled a collective of diverse education experts to craft and deliver localized solutions that teachers could incorporate into their practice. We conclude by reflecting on the efficacy of our intervention in low-resource work contexts and provide recommendations to enhance collective social support interventions similar to Saharaline.

==> drafts/2-literature__copy_if_literature_has_to_be_expanded_in_R_R_.tex <==
\section{Background}

\subsection{Understanding Different Dimensions of Social Support}

\citet{shumaker1984Theory} defined social support as a process of ``exchanging resources'' between individuals where either the provider or the receiver has an explicit intention of improving the well-being of the receiver. Social support has been established as an important buffer for individuals seeking to tackle the problems that are negatively impacting their well-being \cite{lazarus20Stress, Jolly_Kong_Kim_2021}. While these studies were primarily concerned with stressors in one's personal life, subsequent research over the years has revealed similar findings in the context of occupational well-being \cite{}. Specifically within contexts of work, social support can manifest in a myriad of ways, prominent examples being peer support \cite{}, vocational intervention \cite{}, employee assistive programs \cite{}, mentorship and coaching\cite{}. Regardless of their specific manifestations, these social support structures are typically governed by three underlying dimensions \cite{wills1991social,taylor2011social}. The first dimension is the \textit{function} of support in an individual's life \cite{house1981Work}. Support can be \textit{problem-focused}, directed at providing assistance to ``manage or alter the problem causing the stress'' \cite{lazarus1984stress}. This type of support can materialize as informational, receiving different types of recommendations that help with stress-management. It can also be instrumental or tangible, receiving explicit assistance (e.g., demonstrating how-to) to reduce stress. Social support can also be \textit{emotion-focused}, directed at providing support to ``regulate emotional responses to the problem'' \cite{lazarus1984stress}. One such example is support that can provide an individual with emotional warmth and care to reduce their stress \cite{lazarus20Stress}. Other examples include network support, creating a sense of belonging among people with similar interests \cite{Cutrona_Suhr_1992} and esteem support, referring to expressions of ``regard for one's skills and abilities'' \cite{Cutrona_Suhr_1992}. 

Second dimension is how an individual \textit{perceives} and evaluates their social support in work place\cite{sarason1991perceived}. Prior studies have established a strong positive relationship between social support and overall occupational well-being, indicating that perceived social support by individuals helps reduce stress and improve well-being \cite{Park2004,turner1981social}. Third dimension concerns with the \textit{structure} of the overall support determined by how an individual embeds themselves and interacts in different forms of social networks \cite{Chronister_2006, Jolly_Kong_Kim_2021} . As a consequence, the support can be \textit{individualistic}, wherein a person receives one-on-one support from another individual to cope with their stress. A common example for this type of support is therapy and mentorship \fixme{\cite{}}. Alternatively, the support can be \textit{collective}, wherein an individual receives support as a result of cooperation and/or collaboration from multiple people. What sets this structure apart from individualistic support is the combined effort that is undertaken by several support providers in order to provide social support. A common example of this type of social support is collaborative care provided in healthcare \fixme{\cite{}}. There are also instances where both of these type of social support co-occur (e.g., occupational support on forums). In the next few sections, we explore individual and collective social support around work and technology, especially within the teaching profession. Based on the presented literature, we argue how collective support is an effective form social support system for teachers in India to improve occupational wellbeing.


\subsection{Individualistic Social Support: Technology, Work \& Teaching}
Increasing development of internet and everyday technology has created new avenues for individualized social support through online-mediated communications in the form of emails \cite{Hutson_Cowie_2007}, forums \cite{Turner_Grube_Meyers_2001}, (micro-) blogs \cite{rains2011}, and online conversations (e.g., remote therapy) \fixme{\cite{}}. While, early research on online social support has shown contradictory results \cite{kraut1998Social, shaw2002defense}, increase in the ubiquitous devices like smartphones have expanded the opportunities for individuals to seek one-on-one online support through personal and professional networks \cite{han2016}. In particular, technology has become an important facilitator for information \fixme{\cite{Coursaris_Liu_2009}}, emotional, \fixme{\cite{Buis_2008}} and network support \fixme{\cite{Ashley_Long_Rouner_Broadfoot_2011}}. 

Proliferation of these ubiquitous technologies into occupational settings prompted early HCI scholars to explore their role in work contexts by applying established popular theoretical frameworks, broadly (e.g., social exchange theory) \cite{Bakker_Demerouti_2007, halbesleben2010moderating, cropanzano2005social}. However, more recent HCI research have sought more contextual understanding by studying individualistic social support within specific elements of work, such as upskilling \fixme{\cite{Dill2016}}, performance of specific work functions \cite{yvette18, stdis15,broadbent2016intimacy}, and finding new roles \cite{burke2013, radhika2020, Dillahunt21}. This has prompted integration of HCI research with two key sub-fields. The first integration is around vocational rehabilitation, which has engaged in support through sociotechnical vocational intervention that aim to deal with unemployment and re-employment \cite{}. The second integration is specifically focuses on employee wellbeing in organizational contexts, in particular employee assistance program interventions \cite{}.
    
Building on this foundation within HCI research on the topic of social support, the teaching profession has garnered significant attention, given its unique challenges.  Teaching is an emotionally demanding and labor-intensive occupation, often requiring educators to work in isolation (e.g., teaching) within resource-constrained environments \cite{hargreaves1994changing}. Consequently, teachers frequently contend stress and burnout, contributing to substantial attrition rates \cite{Madigan_Kim_2021}. Moreover, with rapid integration of technology in education has introduced technostress as an additional factor fueling burnout \cite{Zhao_Wang_Wu_Dong_2022}. In the wake of COVID-19 pandemic, the transition to a hybrid teaching format has further exacerbated the isolation and stress inherent to the profession. For instance, \citet{Gonzalez_2021} demonstrated that female teachers with limited prior technology experience reported the highest levels of stress. Within Global South, where this research is situated, these challenges are amplified for several reasons. Teachers in this region mainly rely on smartphone technology for teaching purposes, as compared to laptops and desktops in the Global North, due to their affordability and adaptability in resource-constrained teaching environments \cite{varanasi2019, cannanure2020}. Secondly, the smartphones used by teachers are often personal devices employed in work contexts, introducing complexities not encountered by educators primarily utilizing school-based technological infrastructure \cite{varanasi2020}. Third, The COVID-19 pandemic forced teachers, many of whom had limited experience with remote teaching, to embrace hybrid teaching approaches using smartphones \cite{ravi2022}. Early studies indicate how this push has contributed to reduced confidence, burnout, and attrition \cite{varanasi2021Investigatinga}. 

Having adequate social support systems can be a crucial resource for teachers to alleviate their isolation in teaching, focus on their professional development, and improve their occupational well-being \cite{Richard2011}. Prior research in this area has focused on source, type, issues, and impacts of different types of social support. \citet{house1981Work}, in their seminal work, pose this as a crucial question,  ``\textit{who} gives \textit{what} to \textit{whom} regarding \textit{which} issues?''. 


For instance, one strand of research that examined the effectiveness of peer interactions among teachers to facilitate informational, instrumental, and emotional support in online and offline medium, indicating reduction in stress levels of teachers \cite{dewert2003safe, kinman2011emotional, paulus2008can}. Another strand of research studied how traditional support practices (e.g., emotional, instrumental) in offline teaching translated to technology-enabled online peer interactions in the online forums \cite{clarke2014}. Within this research, a pivotal determinant of whether teacher receives such social support is the availability of resources within the school ecosystem \fixme{\cite{}}, underscoring the impact of resource constraints on peer and management-established social support in low-income teaching communities\fixme{\cite{}}. 

For instance, \citet{} found that while smartphones played a crucial role in facilitating social support-seeking among teachers in low-income schools within India, teachers had to establish these support pathways on their own accord. In such settings, formal channels for seeking support from the management were virtually non-existent due to resource constraints. Teachers, well aware of these limitations, often hesitated to approach the management and peers, anticipating rejection when requesting support. In sum, individualistic social support demands significant resources from support providers, including infrastructure and time commitment, making it challenging to implement it in resource constraint environments \cite{}.  


\subsection{Collective Social Support: Community-based Support Practices within Work Settings}
Community-based social support addresses the challenged posed by individualistic social support by distributing the responsibility of providing support across multiple roles within the ecosystem. Through coordination and collaboration among multiple individuals within the same ecosystem, they can provide social support to an individual seeking support, thereby distributing the burden solely placed on the management or a few peers. This form of support has especially become a common practice in emotion labor intensive roles such as that of hospitality industry workers \cite{Huang_Van2018}, health care workers \cite{Tixier2009}, social workers \cite{Matthie2016}, gig workers \cite{Uttarapong_Bonifacio_2022} and teachers \cite{varanasi2020}. With social media communication (e.g., Facebook, WhatsApp) becoming prominent in work spaces, affordance within these virtual communities (e.g., likes, reactions, and emojis) have became vital to increase social connectedness \cite{varanasi2018, Carr_Wohn_Hayes_2016} and provide new pathways for workers to reach out a multiple at once and seek their collaborative support. For instance, \citet{Poon2023} developed a computer-mediated intervention focused on peer-support for home care workers called ``sharing circles''. The intervention allowed workers to leverage storytelling practice to collectively reflect on their home care experiences and support each other. While this form of support in work reduces the burden on the management by involving different roles (such as peer) within the same community, it is challenging in those work contexts where these roles are already overwhelmed by their own jobs and the competition they bring with the role \fixme{\cite{}}. Teaching work is a common example of this issue as overwhelming evidence points to how teachers are overworked, especially in resource constrained communities.

\textit{Collective} social support efforts strive to overcome this issue by leveraging individuals outside the working community who are not impacted by the ecosystem. While this form of support is studied across different occupational and personal settings, the overall research is quite scattered. For this final section, we want to bring three main strands of literature to formally define and situate collective social support in the context of teaching in low-resource communities.

A strand of research that shapes the notion of collective support is the \textit{collaborative care} (sometimes referred to as collective or cooperative care) movement within health care settings. Collaborative care is an innovative way of treating different type of health concerns, primarily mental health, by mobilizing medical and non-medical specialists to provide a cohesive support system for the individual \cite{suh2020}.The basic premise of such an idea is that the collaboration between different actors, such as health and close ties, to provide social support that is tailored to the individual's needs and is sustainable over a long period of time can improve the overall well-being of individuals \cite{Archer_2012}. What makes collaborative support effective is the inclusion of members outside the medical community (e.g., family members) in facilitating support. Such form of collaborative care reduces excessive strain not only on one type of medical resource but also on the overall healthcare system. Within HCI space, recent research has been interested in designing and evaluating technological solutions (e.g., assistive technology solutions) that assist different actors in providing collaborative care for vulnerable populations, such as differently-abled and senior citizens \cite{amy2020, caldeira2017, Soubutts2021, suh2020}.
%However, a key challenge observed by \citet{elaine23} with such technological assistance, such as home health monitoring systems, is that they have tendency to alter the collaborative care networks and associated practices, where the individual receiving social support feels isolated. 

Another strand of research has studied \textit{collective support} in resource constrained environments. Similar to collaborative support, this form of social support engages actors outside the working community to provide social support to reduce stress on the system. A concrete example of this can be seen in school ecosystem in African contexts, where the families and community members of students volunteer to support teachers' limited resources by providing informal education support to their children \cite{Madaio20} This form of collective support involved parents, siblings, relatives, and even neighbors within the community to share the responsibilities of informal teaching, such as teaching and monitoring to build capacity of the children. In the same vein, intermediary practices within the Global South in different work contexts, such as health \cite{rahman2021} and education \cite{varanasi2020}, have explored the scope of intermediary roles in providing collective support to marginalized communities in different capacities. For instance, community healthcare workers in low-income communities took up the role of gatekeepers in online WhatsApp groups to work together with the community to identify potentially harmful misinformation \citet{varanasi2022}.   

Our study aims to expand this nascent understanding of collective social support further in resource constrained work environments, particularly in Global South. Through pilot deployment of Saharaline, a collective social support system for teachers working in low-income Indian schools, we investigated the feasibility of engaging actors from various educational support organizations within the community. Our goal was to foster collaboration among these individuals in providing sustainable social support to teachers. Additionally, in post-pandemic era, it was imperative to understand if such support could be organized and sustained on low-level technologies. These motivations shaped our two key questions of the research:\\
\textbf{RQ2}: \textit{What are the experiences of support organizations in providing collective social support through a hybrid sociotechnical intervention?}\\ 
\textbf{RQ1}: \textit{How do teachers use hybrid collective-support intervention to improve their occupational wellbeing?}


Answers to these questions and the overall success of collective social support initiatives can raise awareness of the pressing need for employee assistance programs to extend beyond traditional organizational settings and cater to professions that necessitate on-location work.

------


https://link.springer.com/content/pdf/10.1023/A:1007535930286.pdf ( listening support, emotional support, emotional chal-
lenge support, reality confirmation support, task appreciation sup-
port, task challenge support, tangible assistance support, and per-
sonal assistance support)

==> drafts/3-methods_before_shrinking.tex <==
\begin{figure*}
 \centering
 \includegraphics[width=0.8\linewidth]{pics/architecture.png}
  \caption{Overview of Sharaline architecture that shows online/offline interactions. (1) Teacher reaches out to the Saharaline through WhatsApp; (2) facilitator on the helpline assigns a caseworker to the teacher; (3) Caseworker reaches out to the teacher; (4) caseworker collects issues \& intimates facilitator; (5) facilitator maps appropriate expert(s) to resolve issues; (6) experts provide solutions \& intimates facilitator; (7) caseworkers delivers the solutions}
  \label{architecture}
\end{figure*}

\section{Methods}
We now describe our IRB-approved research study, covering Saharaline's design, its three-month deployment in low-income schools (March to May 2022), and the demographics of the support providers and the teachers who used Saharaline.  

\subsection{Saharaline Design}

%\subsubsection{Design Rationale}
A key objective of Saharaline was to improve teachers' occupational well-being in low-income schools by providing them with social support structures that conform to their lived experiences and associated challenges and stressors. Support organizations (or educational non-profits) that work with low-income schools to build their capacities at various levels (students, management, parents, or teachers) fulfill this objective effectively. These organizations conduct workshops, seminars, and professional development classes. While none of them specifically targeted teachers' well-being, they were fully aware of the sociotechnical and sociocultural challenges that teachers face in the school setting. Their awareness of teachers' experiences enabled them to better understand their stressors, which traditional support systems may not adequately address.

For instance, a low-income school can have two support organizations working simultaneously, one working to empower the management in improving the school leadership and administrative capacities, while the other organization might work with teachers to improve their pedagogical capacities. These organizations' functions overlap, leading to cooperation and assistance that can be leveraged to provide assistance. At the same time, these organizations have disparate priorities allowing them to bring their unique resources and expertise. Saharaline leverages these complementary collaborative practices to provide collective support to teachers. Involving multiple organizations also reduces the effort that each organization has to invest in providing support. 

Second, fostering collaboration among multiple such support organizations to deliver collective social support fulfills the objective of de-centralizing the expertise, as proposed by \cite{}. This concept challenges the colonial model of knowledge production, wherein expertise often originates from external actors situated on the peripheries of the communities they aim to assist. Our design objective was to identify experts who were not only aware of local teacher-community norms but also respected their distinctive pedagogical and content knowledge, thereby enabling the co-creation of support solutions with the teachers and support organization members.

Third, support organizations also fulfill another objective by reducing power differential among teachers, their peers, and higher management \cite{Pendse_2022}. As support organizations occupied a neutral position outside the conventional hierarchies of the school system, they were uniquely positioned to be a part of teachers' work lives without needing to establish any power relationships. Such a position allowed them to gain trust and engage in intimate conversations, facilitating a more in-depth understanding of their challenges. This unique position and their implicit investment in reducing issues in these schools made them great providers of confidential social support. 

Lastly, we wanted Saharaline service to provide social support in a \textit{sustainable} fashion by establishing care pathways that teachers could easily adopt in their overburdened work schedules \cite{gavade2023}. To achieve this, we aimed to integrate everyday familiar technologies and apps that teachers could use effortlessly. This allowed us to scale the initiative across multiple schools in different communities. We complemented the technological choice with the design of hybrid sociotechnical support practices that could easily accommodate teachers' busy schedules and provide long-term care. This is in line with \cite{Pendse_2022}'s framework promoting the need to take such structural constraints into consideration while designing support interventions. Collective social support at the foundation of Saharaline plays a crucial role in ensuring support that is sustainable.


\subsubsection{Implementation}
The aforementioned principles were used to develop Saharaline as a simple, hybrid helpline on WhatsApp Business to provide on-demand collective social support. WhatsApp is an invaluable tool in low-income schools due to its ease of use and high adoption rate among teachers in India \cite{} and, more broadly, in the Global South \cite{}. The business version of WhatsApp is geared towards organizations, non-profits, and businesses that want to interact with a wider WhatsApp audience. For this purpose, the business version of the app has additional automation features (e.g., scheduled greeting messages, automated replies, predefined shorthand commands) and multi-user management of a single account (by logging into WhatsApp Web). Both these reasons made WhatsApp a perfect platform to deploy the initial version of the Saharaline helpline. The design and implementation of this intervention was a collaborative effort between researchers who studied teacher work practices, three support organizations, and experienced teachers in low-income communities. All stakeholders regularly met to brainstorm on the designs and the implementation plan, following a participatory design method \fixme{\cite{}}. 


The resultant design of the helpline is shown in \fixme{Figure-\ref{architecture}}. Saharaline consisted of four different stakeholders. The first stakeholders were the two \textit{facilitators} (first-author and a support organization personnel) who managed the WhatsApp helpline. When a teacher reached out to the helpline, a facilitator greeted them, took their basic details, and then informed the nearest available caseworker to connect with the teacher. The facilitator also coordinated internal communications to ensure Saharaline provided the overall support in a timely manner. The second stakeholders, which were \fixme{five \textit{case workers}}, then connected with the teachers on behalf of Saharaline to connect and comprehensively record their key stressors impacting their occupational well-being. Caseworkers belonged to the same community as teachers. They worked for support organizations on the ground. They were well aware of the teacher's local contexts, such as the local language and their standing in the community, allowing them to capture the issues in a comprehensive manner. Once they captured the key issue of the teacher, they recorded and shared it with Saharaline, which was then shared with the third type of stakeholders constituting \fixme{four \textit{experts}}. Experts were proficient in their subject matter, such as mental health, pedagogical and content expertise, and educational technologies, and worked at the headquarters of support organizations. These workers understood the issues remotely along with the context shared by the caseworkers and formulated appropriate support solutions that aimed to address teachers' problems. The fourth stakeholder comprised of  \fixme{28 \textit{teachers}}  who reached out and interacted with Saharaline to seek social support for stressful events in their teaching lives. These teachers belonged to affordable private schools and government schools, primarily catering to low-income students.


\subsection{Study Procedure}
Sahraline was implemented for three months across three states in India (starting March 2022). In order to deploy and study the Saharaline intervention, we collaborated with four support organizations. Three organizations that engaged in the design efforts of Saharaline infrastructure also showed interest in being part of the intervention study. Additionally, we advertised our efforts to other support organizations working in India through a nationwide mailing list. Out of the five organizations that responded, we shortlisted one. This brought the total number of support organizations to four, allowing us to keep the scope of the intervention study manageable. To deploy Saharaline, we shortlisted six schools in different communities where at least two of the four organizations had a presence. This requirement encouraged support organizations to be organically invested in supporting the teachers while they carried out their usual activities. After receiving approval in six schools, support organization personnel, along with the first author, introduced Saharaline in the schools and periodically shared it in their official WhatsApp groups during the entire period of the study.

\subsubsection{Support Protocol}
To avail support, teachers could reach Saharaline's advertised number through WhatsApp call or message seven days a week between 8 A.M. and 8 P.M. during the three months of deployment. Ensuring daily operation gave teachers the time and flexibility to interact with the Saharaline service in their free time. Upon establishing a connection with the helpline (step-1 in fig \ref{workflow}), the teacher was greeted with an automated message that welcomed them to the helpline and provided them with a template to provide the basic details, such as their demographics and the issue overview. Based on the details, the facilitator operating Saharaline forwarded the details to the appropriate caseworker in the community (step-2). 

The caseworker, in turn, reached out to the teacher and inquired about their issues comprehensively (step-3). To accommodate the teachers' busy work schedule, the caseworkers provided multiple interaction options, offline or online, before or after school hours. Based on the teacher's preference, the caseworker found the time and location to capture the teacher's well-being levels, persona, working ecosystem, standing with the management and peers, and a key problem (stressor) for which the teacher needed support. They captured this information in a document called \textit{case file} and submitted it to Saharaline number in response (step-4). The case file had a semi-structured template with category placeholders for and guiding question  

Based on the problem registered by the caseworker, the facilitators handling Saharaline then routed the case to the appropriate expert (step-5). For instance, if the key stressor for the teacher was not being able to find strategies to teach a classroom with varied learning levels post-pandemic, it was routed to the teacher expert to provide pedagogical support. In addition to teacher experts who provided pedagogical and content support, Saharaline also constituted a mental health expert specializing in occupational well-being and an expert specializing in education technologies. When a particular case overlapped with multiple experts, the case file was routed parallelly to multiple experts. Experts used the information in the case file to understand the teacher's persona. In case of gaps in the case file, the expert reached out to the helpline with queries, which facilitators routed to the caseworker for clarification. The caseworker's responses were then provided back to the expert. Accordingly, experts created a list of solutions, resources, and directions for the teacher that addressed their reported problem, appending them to the case file (step-6). Over a period, the case file contained all issues and support advice given to teachers across multiple visits.

Once the experts added the solutions, the facilitator informed the caseworker to convey the solutions to the teacher. The caseworker then scheduled a follow-up appointment with the teacher to meaningfully explain the solutions provided by the experts. A typical time between the teacher reaching out to Saharaline and receiving social support was about seven days (see ref \ref{workflow}). This cycle allowed the caseworker to handle multiple cases daily while managing their usual support work. In order to implement Sarahaline's longitudinal social support,  caseworkers reached out to the teacher a few days after providing the solution to take feedback and inquire if there were any other issues where the teacher required support. Saharaline repeated the support cycle if the teacher asked follow-up questions or shared a new problem.


\subsubsection{Participant Demography}
The six schools comprised \fixme{73} teachers. The first two schools were located in a remote community in the Northeast state of Meghalaya. Both schools were government-sponsored and catered to low-income communities. The two support organizations working in the schools engaged with teachers and higher management. The second set of two schools were low-income private schools in the semi-urban community of Gujarat. Support organizations working in these schools focused on students and higher management. The last set of two schools was in urban communities in Karnataka, where support organizations were exclusively working with teachers. All six schools were fully functional offline and were operational post-COVID-19. Out of the \fixme{28} teachers who used Saharaline, \fixme{16} were teaching primary classes while \fixme{12} were teaching secondary schools. 

The five caseworkers were distributed across the six schools, with two caseworkers in Karnataka and Meghalaya and one in Gujarat. The caseworkers worked as support personnel in different organizations for an average duration of \fixme{two years} before participating in the intervention. They also lived close to the schools where they provided support. All five caseworkers were graduates. Three of them were women, while two were men. The average age of the caseworkers was 26 years. The four experts were part of the three different support organizations, with an average experience of \fixme{3.5 years} in teacher training, designing educational content, developing educational technologies, and practicing occupational therapy, respectively. Three of them were post-graduates, while one had a doctoral degree. Three of the four experts were women. All four experts were in the cities where the organization's headquarters were. Finally, the average age of the experts was 35 years. 

\subsection{Data Collection \& Analysis}
Saharaline intervention produced three types of data that we analyzed to understand the teachers' and support providers' overall support experiences. The first set of data consisted of 28 case files created for each teacher who contacted the helpline. The case file contained teachers' demographics, their persona, and a log of caseworkers' observations of the teachers' issues. The case file also contained solutions comprising representative examples with different embedded (or links) images and videos about teaching-learning materials and pedagogical materials  \fixme{(appendix for a sample case file)}. These files painted a concrete picture of the support providers' perspectives during various stages of social support. %example.

The second data set was the recorded interactions between teachers, caseworkers, and experts as part of the support effort. These interactions included WhatsApp texts and audio messages that captured (1) initial messages that teachers reached out with when they shared their issues, (2) the caseworkers' interaction with the teachers through WhatsApp messages for coordination, clarification, and solution sharing (3) and interactions between the caseworkers and the experts for purposes of coordination and follow-up clarification. Within this category, we obtained \fixme{432} messages between the three stakeholders. We exported all the messages after receiving explicit permission. We also analyzed the interactions the caseworkers recorded when they met the teachers in-person.

The third set of data came in the form of interviews that the first author conducted with the caseworkers, experts, and teachers to capture their overall support-providing and seeking experiences once the intervention was over. In total, we obtained \fixme{75 hours} of interviews and conversational audio recordings. Lastly, we also collected 21 pages of detailed notes from the first author of observations while managing the helpline. Analyzing different forms of data allowed us to triangulate \cite{cresswell} and establish a strong sense of validity for our findings. 

We started the analysis by translating the data captured in local languages, Hindi, and Kannada into English. After that, we engaged in qualitative coding using inductive thematic analysis \cite{terry2017thematic}. The process began with us taking multiple passes of all of our data to internalize the different accounts and perspectives. For the artifacts and messages, we began by going through the logs, similar to \cite{varanasi2021Tag}, to conduct multiple rounds of open coding. Our unit of analysis was a single message sent by an individual participant. If the participant broke the message in multiple lines, we treated it as a single message. We avoided any pre-conceived notions and instead allowed the codes and categories to emerge from the participants' data. A similar analysis approach was taken for the interviews. A second layer of internal validity was achieved with the data through peer debriefing \cite{creswell} by multiple researchers, both external and internal to the intervention study. Our analysis resulted in \fixme{77} codes (e.g., \fixme{``\textit{sources of tension}''}, \fixme{``\textit{material assistance}''}, \fixme{``\textit{meta explaination for caseworkers}''}). The overall codes were translated into \fixme{nine} themes (e.g., \fixme{``\textit{Caseworker assistance in problem capture}''}, \fixme{``\textit{Contextual followups for teachers}''}, \fixme{``\textit{Expert Clarifications}''}).  




